On the Transferability of Visual Features in Generalized Zero-Shot Learning

Generalized Zero-Shot Learning (GZSL) aims to train a classifier that can generalize to unseen classes, using a set of attributes as auxiliary information, and the visual features extracted from a pre-trained convolutional neural network. While recent GZSL methods have explored various techniques to leverage the capacity of these features, there has been an extensive growth of representation learning techniques that remain under-explored. In this work, we investigate the utility of different GZSL methods when using different feature extractors, and examine how these models' pre-training objectives, datasets, and architecture design affect their feature representation ability. Our results indicate that 1) methods using generative components for GZSL provide more advantages when using recent feature extractors; 2) feature extractors pre-trained using self-supervised learning objectives and knowledge distillation provide better feature representations, increasing up to 15% performance when used with recent GZSL techniques; 3) specific feature extractors pre-trained with larger datasets do not necessarily boost the performance of GZSL methods. In addition, we investigate how GZSL methods fare against CLIP, a more recent multi-modal pre-trained model with strong zero-shot performance. We found that GZSL tasks still benefit from generative-based GZSL methods along with CLIP's internet-scale pre-training to achieve state-of-the-art performance in fine-grained datasets. We release a modular framework for analyzing representation learning issues in GZSL here: https://github.com/uvavision/TV-GZSL

==> 04.3_subset_table_AWA2_noclip.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\midrule
\multicolumn{17}{@{\hskip 0.11in}c}{\bf {AWA2 Dataset}}  \\
\midrule

\multirow{6}{*}{I-1k} & &
\multirow{3}{*}{CNN\cite{Alexnet}} & &
RN101\cite{RNs} &&
71.78 & 17.30 & 27.88 & &
88.84 & 4.04 & 7.72 & &
77.59 & 12.15 & 21.01  \\ 

&& &&RN101\cite{RNs}+FT &&
87.34 & 18.83 & 30.99 & &
93.07 & 6.12 & 11.49 & &
92.64 & 8.25 & 15.16  \\ 

% && &&GoogleNet &&
% 68.56 & 17.40 & 27.76 & &
% 80.11 & 4.26 & 8.10 & &
% 82.82 & 5.13 & 9.66  \\ 

&& &&\cellcolor{gray!18}RN152\cite{RNs} &\cellcolor{gray!18}&
\cellcolor{gray!18}88.30 & \cellcolor{gray!18}\textbf{21.18} & \cellcolor{gray!18}\textbf{34.17} & &
91.31 & 5.94 & 11.15 & &
85.46 & 12.91 & 22.43  \\ 


% && &&Inceptionv3$_{\text{adv}}$ &&
% 89.33 & 12.14 & 21.38 & &
% 91.69 & 3.53 & 6.79 & &
% 82.21 & 8.06 & 14.69  \\ 

% \cmidrule{5-17}
% && &&RN50-MOCO$^{\dag}$ &&
% 78.23 & 11.07 & 19.39 & &
% 57.62 & 3.73 & 7.01 & &
% 81.51 & 4.60 & 8.71  \\ 

% \cmidrule{3-17}

% && MLP&&MLP-Mixer && 
% 21.06 & 10.87 & 14.34 && 
% 38.51 & 2.67 & 4.99 && 
% 94.29 & 12.78 & 22.52  \\ 

\cmidrule{3-17}

&& \multirow{2}{*}{ViT}\cite{ViT} &&\cellcolor{gray!18}ViT$_{\text{large}}$\cite{ViT_21k}&\cellcolor{gray!18}&
83.78 & 18.00 & 29.63 &\cellcolor{gray!18}& 
\cellcolor{gray!18}\textbf{97.07} & \cellcolor{gray!18}\textbf{18.62} & \cellcolor{gray!18}\textbf{31.25} & &
92.28 & 13.75 & 23.93  \\

&& &&\cellcolor{gray!18}DeiT$_{\text{base}}$\cite{DeiT} &\cellcolor{gray!18}& 
\textbf{91.41} & 9.51 & 17.22 & &
94.08 & 2.33 & 4.54 &\cellcolor{gray!18} &
\cellcolor{gray!18}87.37 & \cellcolor{gray!18}\textbf{14.67} & \cellcolor{gray!18}\textbf{25.12}  \\ 

&& &&ViTB16-DINO$^{\dag}$&& 
71.83 & 19.41 & 30.56 & &
92.34 & 5.08 & 9.63 & &
79.73 & 6.55 & 12.10  \\ 

\midrule

% \multirow{2}{*}{I-21k}
% && MLP && 
% MLP-Mixer$_{\text{L16}}$ & &
% 82.92 & 10.37 & 18.43 & &
% 85.48 & 1.47 & 2.90 & &
% 86.24 & 1.88 & 3.69  \\ 

% \cmidrule{3-17}

% && \multirow{3}{*}{ViT} && ViT$_{\text{base}}$ & &
% 82.35 & 14.05 & 24.00 & &
% 96.18 & 7.77 & 14.38 & &
% \textbf{95.62} & 11.07 & 19.85  \\ 

I-21k && ViT\cite{ViT} && ViT$_{\text{large}}$\cite{ViT_21k} & &
86.49 & 19.53 & 31.87 & &
96.47 & 10.43 & 18.83 & &
95.03 & 12.76 & 22.49  \\ 

&& && ViT$_{\text{huge}}$ & &
80.00 & 12.37 & 21.43 & &
89.57 & 2.55 & 4.95 & &
81.40 & 6.72 & 12.41  \\ 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> 04.3_subset_table_CUB_noclip.tex <==
\begin{table*}[ht!]
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}
\newcolumntype{Z}{>{\centering\arraybackslash}X}
\centering
\footnotesize
\setlength\tabcolsep{1pt}
\renewcommand{\arraystretch}{1.2}

\scalebox{0.87}{

\begin{tabularx}{\textwidth}{l c l c l c YYY c YYY c YYY}
\toprule

% \multicolumn{17}{@{\hskip 0.11in}c}{\bf \shortstack{Embedding Based GZSL Methods\\ CUB\cite{CUB} Dataset}}  \\
\multicolumn{17}{@{\hskip 0.11in}c}{\bf {CUB Dataset}}  \\
\midrule

{\multirow{2}{*}{\bf \shortstack{Dataset\\Pret. on}}}~ &~~~&
{\multirow{2}{*}{\bf \shortstack{Arch\\ Type}}}~ &~~&
{\multirow{2}{*}{\bf Backbone}}~ &~~&
\multicolumn{3}{@{\hskip 0.11in}c}{\bf DEVISE} &~~~~& 
\multicolumn{3}{@{\hskip 0.11in}c}{\bf ESZSL} &~~~~& 
\multicolumn{3}{@{\hskip 0.11in}c}{\bf ALE} \\

\cmidrule{7-9}\cmidrule{11-13}\cmidrule{15-17}

&& && && \textit{Seen} & \textit{Novel} & \textit{Harm.} 
&& \textit{Seen} & \textit{Novel} & \textit{Harm.} 
&& \textit{Seen} & \textit{Novel} & \textit{Harm.} \\

\midrule

\multirow{5}{*}{I-1k} & &
\multirow{2}{*}{CNN} & &
RN101 &  & 
61.96 & 23.41 & 33.98 &&
56.53 & 14.70 & 23.34 &&
62.74 & 26.07 & 36.83 \\ 

&& && RN101+FT &  & 
83.42 & 28.32 & 42.28 &&
81.45 & 16.14 & 26.94 &&
83.04 & 30.36 & 44.46 \\ 

&& && GoogleNet &  &  
35.57 & 15.10 & 21.20 && 
30.79 & 9.70 & 14.75 && 
36.86 & 17.67 & 23.89  \\ 

&& && RN152 &  &  
45.73 & 19.01 & 26.86 &&
46.39 & 15.49 & 23.23 &&
52.69 & 24.84 & 33.76  \\ 

\cmidrule{3-17}

&& \multirow{3}{*}{ViT} &&ViT$_{\text{large}}$&&
71.85 & 23.88 & 35.85 & &
\textbf{83.64} & 12.26 & 21.39  & &
72.20 & 23.44 & 35.39  \\

&& &&DeiT$_{\text{base}}$ && 
70.45 & 25.86 & 37.83 & &
60.88 & 16.81 & 26.35  & &
73.88 & 30.88 & 43.55  \\  

&& &&\cellcolor{gray!18}ViTB16-DINO$^{\dag}$&\cellcolor{gray!18}& 
75.50 & \textbf{32.20} & 45.15 &\cellcolor{gray!18} &
\cellcolor{gray!18}70.89 & \cellcolor{gray!18}\textbf{29.06} & \cellcolor{gray!18}\textbf{41.23}  & &
77.21 & \textbf{36.83} & 49.87  \\ 

\midrule

&& && ViT$_{\text{large}}$ & &
\textbf{85.24} & 25.61 & 39.38 & &
82.47 & 17.53 & 28.92 & &
83.09 & 22.08 & 34.89  \\ 

\multirow{1}{*}{I-21k} && {ViT} && \cellcolor{gray!18}ViT$_{\text{huge}}$ &\cellcolor{gray!18} &
\cellcolor{gray!18}82.78 & \cellcolor{gray!18}31.31 & \cellcolor{gray!18}\textbf{45.44} & &
61.88 & 18.77 & 28.80 &\cellcolor{gray!18} &
\cellcolor{gray!18}\textbf{84.00} & \cellcolor{gray!18}36.05 & \cellcolor{gray!18}\textbf{50.45}  \\ 

\midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\multirow{2}{*}{\bf \shortstack{ }}}~ &~~~~&
{\multirow{2}{*}{\bf \shortstack{ }}}~ &~~~~&
{\multirow{2}{*}{\bf  }}~ &~~~~&
\multicolumn{3}{@{\hskip 0.11in}c}{\bf tfVAEGAN} &~~~~& 
\multicolumn{3}{@{\hskip 0.11in}c}{\bf CADA-VAE} &~~~~& 
\multicolumn{3}{@{\hskip 0.11in}c}{\bf CE} \\

\cmidrule{7-9}\cmidrule{11-13}\cmidrule{15-17}

&& && && \textit{Seen} & \textit{Novel} & \textit{Harm.} 
&& \textit{Seen} & \textit{Novel} & \textit{Harm.} 
&& \textit{Seen} & \textit{Novel} & \textit{Harm.} \\

\midrule

\multirow{3}{*}{I-1k} & &
\multirow{2}{*}{CNN} & &


RN101 &&
57.08 & 42.88 & 48.97 &&
58.27 & 49.71 & 53.65  &&
60.09 & \textbf{49.05} & 54.01  \\ 

&& &&\cellcolor{gray!18}RN101+FT &\cellcolor{gray!18}&
72.44 & 53.66 & 61.65 &&
76.45 & 57.53 & 65.65  &&
\cellcolor{gray!18}\textbf{76.71} &\cellcolor{gray!18} 48.81 &\cellcolor{gray!18} \textbf{59.66}  \\  

&& &&GoogleNet &&
38.54 & 33.34 & 35.76 &&
33.84 & 30.20 & 31.92  &&
33.72 & 26.05 & 29.39  \\ 

&& &&RN152 &&
50.23 & 44.48 & 47.18 &&
47.58 & 41.64 & 44.41  &&
45.77 & 35.52 & 40.00  \\ 

\cmidrule{3-17}

&& \multirow{1}{*}{ViT} &&ViT$_{\text{large}}$&&
\textbf{80.34} & 54.34 & 64.83 &&
61.23 & 53.31 & 56.99  &&
70.22 & 43.07 & 53.39  \\

&& &&DeiT$_{\text{base}}$ && 
73.29 & 49.44 & 59.05 &&
60.39 & 50.05 & 54.74  &&
55.68 & 38.68 & 45.65  \\  

&& &&ViTB16-DINO$^{\dag}$&& 
76.82 & 57.94 & 66.06 &&
71.95 & 55.37 & 62.58  &&
61.29 & 45.47 & 52.21  \\

\midrule

\multirow{2}{*}{I-21k} && \multirow{2}{*}{ViT} &&
ViT$_{\text{large}}$ & &
76.95 & 61.56 & 68.40 &&
72.54 & 58.94 & 65.04  &&
67.16 & 46.94 & 55.26  \\ 

% \multirow{2}{*}{I-21k} && \multirow{2}{*}{ViT} && ViT$_{\text{huge}}$ & &
% 75.15 & 62.76 & 68.40 &&
% 70.53 & 60.50 & 65.13  &&
% 49.37 & 43.76 & 46.40  \\

&& &&\cellcolor{gray!18} ViT$_{\text{huge}}$+FT &\cellcolor{gray!18} &
\cellcolor{gray!18}78.32 &\cellcolor{gray!18} \textbf{76.26} &\cellcolor{gray!18} \textbf{77.27} &\cellcolor{gray!18}&
\cellcolor{gray!18}\textbf{77.99} &\cellcolor{gray!18} \textbf{74.46} &\cellcolor{gray!18} \textbf{76.18}  &&
70.87&	44.66 &	54.79 \\

\midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\multirow{2}{*}{\bf \shortstack{ }}}~ &~~~~&
{\multirow{2}{*}{\bf \shortstack{ }}}~ &~~~~&
{\multirow{2}{*}{\bf  }}~ &~~~~&
\multicolumn{3}{@{\hskip 0.11in}c}{\bf SDGZSL} &~~~~& 
\multicolumn{3}{@{\hskip 0.11in}c}{\bf FREE}  \\

\cmidrule{7-9}\cmidrule{11-13}

&& && && \textit{Seen} & \textit{Novel} & \textit{Harm.} 
&& \textit{Seen} & \textit{Novel} & \textit{Harm.} \\

\midrule

\multirow{3}{*}{I-1k} & &
\multirow{2}{*}{CNN} & &

RN101 &&
56.41 & 51.89 & 54.06  & ~ &
58.30 & 55.10 & 56.70  \\

&& &&RN101+FT &&
75.00 & 64.26 & 69.21  & ~ &
75.30 & 56.00 & 64.20  \\

&& &&GoogleNet &&
32.72 & 32.88 & 32.80  & ~ &
33.78 & 34.34 & 34.06  \\

&& &&RN152 &&
48.22 & 43.37 & 45.67  & ~ &
50.70 & 43.90 & 47.10  \\

\cmidrule{3-13}

&& \multirow{3}{*}{ViT} &&ViT$_{\text{large}}$&&
74.17 & 63.17 & 68.23  & ~ &
69.53 & 56.38 & 62.27  \\

&& &&DeiT$_{\text{base}}$ && 
62.91 & 54.40 & 58.35  & ~ &
61.80 & 43.80 & 51.27  \\ 

&& &&ViTB16-DINO$^{\dag}$&& 
68.72 & 64.25 & 66.41  & ~ &
73.70 & 53.46 & 61.97  \\

\midrule

\multirow{2}{*}{I-21k} && \multirow{2}{*}{ViT} && 
ViT$_{\text{large}}$ & &
79.55 & 64.37 & 71.16  & ~ &
73.07 & 52.91 & 61.37  \\

&& &&\cellcolor{gray!18} ViT$_{\text{huge}}$+FT &\cellcolor{gray!18} &
\cellcolor{gray!18}\textbf{79.68} &\cellcolor{gray!18} \textbf{73.27} &\cellcolor{gray!18} \textbf{76.34}  &\cellcolor{gray!18} ~ &
\cellcolor{gray!18}\textbf{80.57} &\cellcolor{gray!18} \textbf{69.71} &\cellcolor{gray!18} \textbf{74.75}  \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bottomrule
\end{tabularx}

}


%\vspace{-0.05in}
\caption{
 
Results of Generative Based Methods using different features extracted from a diverse set of architecture types pretrained on ImageNet-1k (I-1k) and ImageNet-21k (I-21k). (${\dag}$) indicates self-supervised learning. The bold numbers and the shaded rows correspond to the highest scores and method. +FT indicates the features were fine-tuned with the seen classes from the training set. 
}
\label{tab:subset_embedding_based}
% \vspace{-0.2in}
\end{table*}

==> 04.3_subset_table_SUN_noclip.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\midrule
\multicolumn{17}{@{\hskip 0.11in}c}{\bf {SUN Dataset}}  \\
\midrule

\multirow{5}{*}{I-1k} & &
\multirow{2}{*}{CNN\cite{Alexnet}} & &
RN101\cite{RNs} & &
32.75 & 18.54 & 23.68 && 
28.41 & 13.75 & 18.53 && 
37.13 & 23.68 & 28.92  \\ 

&& &&RN101\cite{RNs}+FT &  &
34.03 & 19.93 & 25.14 && 
33.18 & 13.82 & 19.51 && 
37.95 & 22.43 & 28.19  \\ 

% && &&GoogleNet & &
% 18.02 & 10.83 & 13.53 && 
% 17.52 & 9.31 & 12.15 && 
% 24.88 & 15.76 & 19.30  \\ 

&& &&RN152 & &
30.39 & 17.29 & 22.04 && 
26.63 & 15.90 & 19.91 && 
35.70 & 23.40 & 28.27  \\ 

% && &&Inceptionv3 & &
% 31.01 & 14.03 & 19.32 && 
% 25.08 & 11.25 & 15.53 && 
% 32.29 & 18.47 & 23.50  \\ 

% && &&Inceptionv3$_{\text{adv}}$ & &
% 27.91 & 15.00 & 19.51 && 
% 24.69 & 12.08 & 16.23 && 
% 33.88 & 21.39 & 26.22  \\ 

% \cmidrule{5-17}
% && &&RN50-MOCO$^{\dag}$ & &
% 2.25 & 0.00 & 0.00 && 
% 3.14 & 3.33 & 3.23 && 
% 34.92 & 23.33 & 27.98  \\ 

% \cmidrule{3-17}

% && MLP&&MLP-Mixer && 
% 6.32 & 3.33 & 4.36 & &
% 6.40 & 2.36 & 3.45 & &
% 8.29 & 3.96 & 5.36  \\

\cmidrule{3-17}

&& \multirow{1}{*}{ViT}\cite{ViT} &&\cellcolor{gray!18}ViT$_{\text{large}}$\cite{ViT_21k}&\cellcolor{gray!18}&
\textbf{52.33} & 24.51 & 33.39 && 
\textbf{44.84} & 18.82 & 26.51 &\cellcolor{gray!18} &
\cellcolor{gray!18}\textbf{59.77} &\cellcolor{gray!18} \textbf{34.10} & \cellcolor{gray!18}\textbf{43.42}  \\

&& &&DeiT$_{\text{base}}$ && 
37.17 & 17.22 & 23.54 & &
28.49 & 12.57 & 17.44 & &
38.37 & 21.53 & 27.58  \\ 

&& &&ViTB16-DINO$^{\dag}$&& 
35.19 & 20.97 & 26.28 & &
32.48 & 16.11 & 21.54 & &
40.89 & 28.40 & 33.52  \\ 

\midrule

% \multirow{2}{*}{I-21k}
% && MLP && 
% MLP-Mixer$_{\text{L16}}$ & &
% 24.57 & 11.18 & 15.37 & &
% 20.74 & 9.24 & 12.78 & &
% 29.03 & 13.61 & 18.53  \\ 

% \cmidrule{3-17}

% && \multirow{3}{*}{ViT} && ViT$_{\text{base}}$ & &
% 45.19 & 25.07 & 32.25 & &
% 40.43 & 19.51 & 26.32 & &
% 52.87 & 31.81 & 39.72  \\ 

\multirow{1}{*}{I-21k} && ViT\cite{ViT} && \cellcolor{gray!18}ViT$_{\text{large}}$\cite{ViT_21k} &\cellcolor{gray!18} &
\cellcolor{gray!18}49.15 &\cellcolor{gray!18} \textbf{25.56} &\cellcolor{gray!18} \textbf{33.63} &\cellcolor{gray!18} &
\cellcolor{gray!18}43.29 &\cellcolor{gray!18} \textbf{19.86} &\cellcolor{gray!18} \cellcolor{gray!18}\textbf{27.23} & &
55.23 & 33.26 & 41.52  \\ 

&& && ViT$_{\text{huge}}$ & &
38.22 & 19.24 & 25.59 & &
31.71 & 18.13 & 23.06 & &
51.55 & 30.07 & 37.98  \\ 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> 04.3_subset_tables_embedding_noclip.tex <==
\begin{table*}[ht!]
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}
\newcolumntype{Z}{>{\centering\arraybackslash}X}
\centering
\footnotesize
\setlength\tabcolsep{1pt}
\renewcommand{\arraystretch}{1.2}

\scalebox{0.87}{

\begin{tabularx}{\textwidth}{l c l c l c YYY c YYY c YYY}
\toprule

% \multicolumn{17}{@{\hskip 0.11in}c}{\bf \shortstack{Embedding Based GZSL Methods\\ CUB\cite{CUB} Dataset}}  \\
\multicolumn{17}{@{\hskip 0.11in}c}{\bf {CUB Dataset}}  \\
\midrule

{\multirow{2}{*}{\bf \shortstack{Dataset\\Pret. on}}}~ &~~~&
{\multirow{2}{*}{\bf \shortstack{Arch\\ Type}}}~ &~~&
{\multirow{2}{*}{\bf Backbone}}~ &~~&
\multicolumn{3}{@{\hskip 0.11in}c}{\bf DEVISE\cite{DeViSE}} &~~~~& 
\multicolumn{3}{@{\hskip 0.11in}c}{\bf ESZSL\cite{ESZSL}} &~~~~& 
\multicolumn{3}{@{\hskip 0.11in}c}{\bf ALE\cite{ALE}} \\

\cmidrule{7-9}\cmidrule{11-13}\cmidrule{15-17}

&& && && \textit{Seen} & \textit{Novel} & \textit{Harm.} 
&& \textit{Seen} & \textit{Novel} & \textit{Harm.} 
&& \textit{Seen} & \textit{Novel} & \textit{Harm.} \\

\midrule

\multirow{5}{*}{I-1k} & &
\multirow{2}{*}{CNN} & &
RN101 &  & 
61.96 & 23.41 & 33.98 &&
56.53 & 14.70 & 23.34 &&
62.74 & 26.07 & 36.83 \\ 

&& && RN101+FT &  & 
83.42 & 28.32 & 42.28 &&
81.45 & 16.14 & 26.94 &&
83.04 & 30.36 & 44.46 \\ 

% && && GoogleNet\cite{Googlenet} &  &  
% 35.57 & 15.10 & 21.20 && 
% 30.79 & 9.70 & 14.75 && 
% 36.86 & 17.67 & 23.89  \\ 

&& && RN152 &  &  
45.73 & 19.01 & 26.86 &&
46.39 & 15.49 & 23.23 &&
52.69 & 24.84 & 33.76  \\ 

% && && Inceptionv3\cite{inception} &  &  
% 58.09 & 21.81 & 31.71 && 
% 48.30 & 12.91 & 20.38 && 
% 53.11 & 21.52 & 30.63  \\ 

% && && Inceptionv3$_{\text{adv}}$\cite{adv_inception} &  &  
% 54.84 & 20.86 & 30.22 && 
% 47.70 & 11.09 & 18.00 && 
% 59.37 & 20.24 & 30.18  \\ 

% \cmidrule{5-17}
% && && RN50-MOCO$^{\dag}$\cite{MoCo} &  &  
% 31.26 & 11.39 & 16.70 && 
% 7.69 & 3.87 & 5.15 && 
% 32.73 & 15.77 & 21.28  \\ 

% \cmidrule{3-17}

% && MLP\cite{MLPMixer}&&MLP-Mixer\cite{MLPMixer} && 
% 19.17 & 7.76 & 11.05 & &
% 20.50 & 5.53 & 8.71 & &
% 19.82 & 8.11 & 11.51  \\

\cmidrule{3-17}

&& \multirow{3}{*}{ViT} &&ViT$_{\text{large}}$&&
71.85 & 23.88 & 35.85 & &
\textbf{83.64} & 12.26 & 21.39  & &
72.20 & 23.44 & 35.39  \\

&& &&DeiT$_{\text{base}}$\cite{DeiT} && 
70.45 & 25.86 & 37.83 & &
60.88 & 16.81 & 26.35  & &
73.88 & 30.88 & 43.55  \\  

&& &&\cellcolor{gray!18}ViTB16-DINO$^{\dag}$&\cellcolor{gray!18}& 
75.50 & \textbf{32.20} & 45.15 &\cellcolor{gray!18} &
\cellcolor{gray!18}70.89 & \cellcolor{gray!18}\textbf{29.06} & \cellcolor{gray!18}\textbf{41.23}  & &
77.21 & \textbf{36.83} & 49.87  \\ 

\midrule

% \multirow{2}{*}{I-21k}
% && MLP\cite{MLPMixer} && 
% MLP-Mixer$_{\text{L16}}$\cite{MLPMixer} & &
% 38.46 & 12.02 & 18.32 & &
% 34.62 & 5.82 & 9.97 & &
% 41.66 & 10.68 & 17.00  \\

% \cmidrule{3-17}

&& && ViT$_{\text{large}}$ & &
\textbf{85.24} & 25.61 & 39.38 & &
82.47 & 17.53 & 28.92 & &
83.09 & 22.08 & 34.89  \\ 

\multirow{1}{*}{I-21k} && {ViT} && \cellcolor{gray!18}ViT$_{\text{huge}}$ &\cellcolor{gray!18} &
\cellcolor{gray!18}82.78 & \cellcolor{gray!18}31.31 & \cellcolor{gray!18}\textbf{45.44} & &
61.88 & 18.77 & 28.80 &\cellcolor{gray!18} &
\cellcolor{gray!18}\textbf{84.00} & \cellcolor{gray!18}36.05 & \cellcolor{gray!18}\textbf{50.45}  \\ 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\midrule
\multicolumn{17}{@{\hskip 0.11in}c}{\bf {SUN Dataset}}  \\
\midrule

\multirow{5}{*}{I-1k} & &
\multirow{2}{*}{CNN} & &
RN101 & &
32.75 & 18.54 & 23.68 && 
28.41 & 13.75 & 18.53 && 
37.13 & 23.68 & 28.92  \\ 

&& &&RN101+FT &  &
34.03 & 19.93 & 25.14 && 
33.18 & 13.82 & 19.51 && 
37.95 & 22.43 & 28.19  \\ 

% && &&GoogleNet & &
% 18.02 & 10.83 & 13.53 && 
% 17.52 & 9.31 & 12.15 && 
% 24.88 & 15.76 & 19.30  \\ 

&& &&RN152 & &
30.39 & 17.29 & 22.04 && 
26.63 & 15.90 & 19.91 && 
35.70 & 23.40 & 28.27  \\ 

% && &&Inceptionv3 & &
% 31.01 & 14.03 & 19.32 && 
% 25.08 & 11.25 & 15.53 && 
% 32.29 & 18.47 & 23.50  \\ 

% && &&Inceptionv3$_{\text{adv}}$ & &
% 27.91 & 15.00 & 19.51 && 
% 24.69 & 12.08 & 16.23 && 
% 33.88 & 21.39 & 26.22  \\ 

% \cmidrule{5-17}
% && &&RN50-MOCO$^{\dag}$ & &
% 2.25 & 0.00 & 0.00 && 
% 3.14 & 3.33 & 3.23 && 
% 34.92 & 23.33 & 27.98  \\ 

% \cmidrule{3-17}

% && MLP&&MLP-Mixer && 
% 6.32 & 3.33 & 4.36 & &
% 6.40 & 2.36 & 3.45 & &
% 8.29 & 3.96 & 5.36  \\

\cmidrule{3-17}

&& \multirow{1}{*}{ViT} &&\cellcolor{gray!18}ViT$_{\text{large}}$&\cellcolor{gray!18}&
\textbf{52.33} & 24.51 & 33.39 && 
\textbf{44.84} & 18.82 & 26.51 &\cellcolor{gray!18} &
\cellcolor{gray!18}\textbf{59.77} &\cellcolor{gray!18} \textbf{34.10} & \cellcolor{gray!18}\textbf{43.42}  \\

&& &&DeiT$_{\text{base}}$ && 
37.17 & 17.22 & 23.54 & &
28.49 & 12.57 & 17.44 & &
38.37 & 21.53 & 27.58  \\ 

&& &&ViTB16-DINO$^{\dag}$&& 
35.19 & 20.97 & 26.28 & &
32.48 & 16.11 & 21.54 & &
40.89 & 28.40 & 33.52  \\ 

\midrule

% \multirow{2}{*}{I-21k}
% && MLP && 
% MLP-Mixer$_{\text{L16}}$ & &
% 24.57 & 11.18 & 15.37 & &
% 20.74 & 9.24 & 12.78 & &
% 29.03 & 13.61 & 18.53  \\ 

% \cmidrule{3-17}

% && \multirow{3}{*}{ViT} && ViT$_{\text{base}}$ & &
% 45.19 & 25.07 & 32.25 & &
% 40.43 & 19.51 & 26.32 & &
% 52.87 & 31.81 & 39.72  \\ 

\multirow{1}{*}{I-21k} && ViT && \cellcolor{gray!18}ViT$_{\text{large}}$ &\cellcolor{gray!18} &
\cellcolor{gray!18}49.15 &\cellcolor{gray!18} \textbf{25.56} &\cellcolor{gray!18} \textbf{33.63} &\cellcolor{gray!18} &
\cellcolor{gray!18}43.29 &\cellcolor{gray!18} \textbf{19.86} &\cellcolor{gray!18} \cellcolor{gray!18}\textbf{27.23} & &
55.23 & 33.26 & 41.52  \\ 

&& && ViT$_{\text{huge}}$ & &
38.22 & 19.24 & 25.59 & &
31.71 & 18.13 & 23.06 & &
51.55 & 30.07 & 37.98  \\ 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\midrule
\multicolumn{17}{@{\hskip 0.11in}c}{\bf {AWA2 Dataset}}  \\
\midrule

\multirow{6}{*}{I-1k} & &
\multirow{3}{*}{CNN} & &
RN101 &&
71.78 & 17.30 & 27.88 & &
88.84 & 4.04 & 7.72 & &
77.59 & 12.15 & 21.01  \\ 

&& &&RN101+FT &&
87.34 & 18.83 & 30.99 & &
93.07 & 6.12 & 11.49 & &
92.64 & 8.25 & 15.16  \\ 

% && &&GoogleNet &&
% 68.56 & 17.40 & 27.76 & &
% 80.11 & 4.26 & 8.10 & &
% 82.82 & 5.13 & 9.66  \\ 

&& &&\cellcolor{gray!18}RN152 &\cellcolor{gray!18}&
\cellcolor{gray!18}88.30 & \cellcolor{gray!18}\textbf{21.18} & \cellcolor{gray!18}\textbf{34.17} & &
91.31 & 5.94 & 11.15 & &
85.46 & 12.91 & 22.43  \\ 


% && &&Inceptionv3$_{\text{adv}}$ &&
% 89.33 & 12.14 & 21.38 & &
% 91.69 & 3.53 & 6.79 & &
% 82.21 & 8.06 & 14.69  \\ 

% \cmidrule{5-17}
% && &&RN50-MOCO$^{\dag}$ &&
% 78.23 & 11.07 & 19.39 & &
% 57.62 & 3.73 & 7.01 & &
% 81.51 & 4.60 & 8.71  \\ 

% \cmidrule{3-17}

% && MLP&&MLP-Mixer && 
% 21.06 & 10.87 & 14.34 && 
% 38.51 & 2.67 & 4.99 && 
% 94.29 & 12.78 & 22.52  \\ 

\cmidrule{3-17}

&& \multirow{2}{*}{ViT} &&\cellcolor{gray!18}ViT$_{\text{large}}$&\cellcolor{gray!18}&
83.78 & 18.00 & 29.63 &\cellcolor{gray!18}& 
\cellcolor{gray!18}\textbf{97.07} & \cellcolor{gray!18}\textbf{18.62} & \cellcolor{gray!18}\textbf{31.25} & &
92.28 & 13.75 & 23.93  \\

&& &&\cellcolor{gray!18}DeiT$_{\text{base}}$\cite{DeiT} &\cellcolor{gray!18}& 
\textbf{91.41} & 9.51 & 17.22 & &
94.08 & 2.33 & 4.54 &\cellcolor{gray!18} &
\cellcolor{gray!18}87.37 & \cellcolor{gray!18}\textbf{14.67} & \cellcolor{gray!18}\textbf{25.12}  \\ 

&& &&ViTB16-DINO$^{\dag}$&& 
71.83 & 19.41 & 30.56 & &
92.34 & 5.08 & 9.63 & &
79.73 & 6.55 & 12.10  \\ 

\midrule

% \multirow{2}{*}{I-21k}
% && MLP && 
% MLP-Mixer$_{\text{L16}}$ & &
% 82.92 & 10.37 & 18.43 & &
% 85.48 & 1.47 & 2.90 & &
% 86.24 & 1.88 & 3.69  \\ 

% \cmidrule{3-17}

% && \multirow{3}{*}{ViT} && ViT$_{\text{base}}$ & &
% 82.35 & 14.05 & 24.00 & &
% 96.18 & 7.77 & 14.38 & &
% \textbf{95.62} & 11.07 & 19.85  \\ 

I-21k && ViT && ViT$_{\text{large}}$ & &
86.49 & 19.53 & 31.87 & &
96.47 & 10.43 & 18.83 & &
95.03 & 12.76 & 22.49  \\ 

&& && ViT$_{\text{huge}}$ & &
80.00 & 12.37 & 21.43 & &
89.57 & 2.55 & 4.95 & &
81.40 & 6.72 & 12.41  \\ 

\bottomrule
\end{tabularx}

}


%\vspace{-0.05in}
\caption{
Results of Embedding Based Methods using different features extracted from a diverse set of architecture types pretrained on ImageNet-1k (I-1k) and ImageNet-21k (I-21k)\cite{Imagenet}. These backbones were trained via: supervised and self-supervised (${\dag}$) learning. The bold numbers correspond to the highest scores per column, and the shaded rows correspond to the most performant image feature per method. +FT indicates the features were fine-tuned with the seen classes from the training set.   
% Results of Generative Based Methods using different features extracted from a diverse set of architecture types pretrained on ImageNet-1k (I-1k) and ImageNet-21k (I-21k). (${\dag}$) indicates self-supervised learning. The bold numbers and the shaded rows correspond to the highest scores and method. +FT indicates the features were fine-tuned with the seen classes from the training set. 
}
\label{tab:subset_embedding_based}
% \vspace{-0.2in}
\end{table*}

==> 04.4_subset_tables_generative_noclip.tex <==
\begin{table*}[ht!]
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}
\newcolumntype{Z}{>{\centering\arraybackslash}X}
\centering
\footnotesize
\setlength\tabcolsep{1pt}
\renewcommand{\arraystretch}{1.2}

\scalebox{0.90}{

\begin{tabularx}{\textwidth}{l c l c l c YYY c YYY c YYY}
\toprule

\multicolumn{17}{@{\hskip 0.11in}c}{\bf {CUB Dataset}}  \\ 
\midrule

{\multirow{2}{*}{\bf \shortstack{Dataset\\Pret. on}}}~ &~~~~&
{\multirow{2}{*}{\bf \shortstack{Arch\\ Type}}}~ &~~~~&
{\multirow{2}{*}{\bf Backbone}}~ &~~~~&
\multicolumn{3}{@{\hskip 0.11in}c}{\bf tfVAEGAN} &~~~~& 
\multicolumn{3}{@{\hskip 0.11in}c}{\bf CADA-VAE} &~~~~& 
\multicolumn{3}{@{\hskip 0.11in}c}{\bf CE} \\

\cmidrule{7-9}\cmidrule{11-13}\cmidrule{15-17}

&& && && \textit{Seen} & \textit{Novel} & \textit{Harm.} 
&& \textit{Seen} & \textit{Novel} & \textit{Harm.} 
&& \textit{Seen} & \textit{Novel} & \textit{Harm.} \\

\midrule

\multirow{3}{*}{I-1k} & &
\multirow{2}{*}{CNN} & &


RN101 &&
57.08 & 42.88 & 48.97 &&
58.27 & 49.71 & 53.65  &&
60.09 & \textbf{49.05} & 54.01  \\ 

&& &&\cellcolor{gray!18}RN101+FT &\cellcolor{gray!18}&
72.44 & 53.66 & 61.65 &&
76.45 & 57.53 & 65.65  &&
\cellcolor{gray!18}\textbf{76.71} &\cellcolor{gray!18} 48.81 &\cellcolor{gray!18} \textbf{59.66}  \\  

% && &&GoogleNet &&
% 38.54 & 33.34 & 35.76 &&
% 33.84 & 30.20 & 31.92  &&
% 33.72 & 26.05 & 29.39  \\ 

&& &&RN152 &&
50.23 & 44.48 & 47.18 &&
47.58 & 41.64 & 44.41  &&
45.77 & 35.52 & 40.00  \\ 

\cmidrule{3-17}

&& \multirow{1}{*}{ViT} &&ViT$_{\text{large}}$&&
\textbf{80.34} & 54.34 & 64.83 &&
61.23 & 53.31 & 56.99  &&
70.22 & 43.07 & 53.39  \\

&& &&DeiT$_{\text{base}}$ && 
73.29 & 49.44 & 59.05 &&
60.39 & 50.05 & 54.74  &&
55.68 & 38.68 & 45.65  \\  

&& &&ViTB16-DINO$^{\dag}$&& 
76.82 & 57.94 & 66.06 &&
71.95 & 55.37 & 62.58  &&
61.29 & 45.47 & 52.21  \\

\midrule

\multirow{2}{*}{I-21k} && \multirow{2}{*}{ViT} &&
ViT$_{\text{large}}$ & &
76.95 & 61.56 & 68.40 &&
72.54 & 58.94 & 65.04  &&
67.16 & 46.94 & 55.26  \\ 

% \multirow{2}{*}{I-21k} && \multirow{2}{*}{ViT} && ViT$_{\text{huge}}$ & &
% 75.15 & 62.76 & 68.40 &&
% 70.53 & 60.50 & 65.13  &&
% 49.37 & 43.76 & 46.40  \\

&& &&\cellcolor{gray!18} ViT$_{\text{huge}}$+FT &\cellcolor{gray!18} &
\cellcolor{gray!18}78.32 &\cellcolor{gray!18} \textbf{76.26} &\cellcolor{gray!18} \textbf{77.27} &\cellcolor{gray!18}&
\cellcolor{gray!18}\textbf{77.99} &\cellcolor{gray!18} \textbf{74.46} &\cellcolor{gray!18} \textbf{76.18}  &&
70.87&	44.66 &	54.79 \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\midrule
\multicolumn{17}{@{\hskip 0.11in}c}{\bf {SUN Dataset}}  \\ 
\midrule

\multirow{3}{*}{I-1k} & &
\multirow{2}{*}{CNN} & &

\cellcolor{gray!18}RN101 &\cellcolor{gray!18}&
38.95 & 45.62 & 42.03  & ~ &
34.15 & 48.96 & 40.23  &\cellcolor{gray!18} ~ &
\cellcolor{gray!18}51.24 &\cellcolor{gray!18} \textbf{55.83} &\cellcolor{gray!18} \textbf{53.44}  \\ 

&& &&RN101+FT &&
35.08 & 38.06 & 36.51  & ~ &
39.84 & 51.60 & 44.97  & ~ &
29.07 & 38.75 & 33.22  \\ 

% && &&GoogleNet &&
% 27.17 & 38.26 & 31.78  & ~ &
% 24.96 & 36.32 & 29.59  & ~ &
% 20.43 & 38.96 & 26.80  \\ 

&& &&RN152 &&
35.35 & 45.97 & 39.97  & ~ &
37.05 & 40.00 & 38.47  & ~ & 26.20 & 43.33 & 32.66  \\ 

\cmidrule{3-17}

&& \multirow{1}{*}{ViT} &&\cellcolor{gray!18}ViT$_{\text{large}}$&\cellcolor{gray!18}&
\cellcolor{gray!18}55.12 &\cellcolor{gray!18} \textbf{64.93} &\cellcolor{gray!18} \textbf{59.62}  &\cellcolor{gray!18} ~ &
\cellcolor{gray!18}\textbf{52.64} &\cellcolor{gray!18} \textbf{61.32} &\cellcolor{gray!18} \textbf{56.65}  & ~ &
50.70 & 52.78 & 51.72  \\

&& &&DeiT$_{\text{base}}$ && 
34.34 & 44.72 & 38.85  & ~ &
37.44 & 44.51 & 40.67  & ~ &
36.36 & 37.57 & 36.95  \\

&& &&ViTB16-DINO$^{\dag}$&& 
42.64 & 52.71 & 47.14  & ~ &
42.52 & 51.18 & 46.45  & ~ &
40.39 & 45.56 & 42.82  \\

\midrule

\multirow{2}{*}{I-21k} && \multirow{2}{*}{ViT} && 
ViT$_{\text{large}}$ & &
\textbf{57.13} & 61.32 & 59.15  & ~ &
52.83 & 60.69 & 56.49  & ~ &
50.12 & 50.69 & 50.40  \\


&& && ViT$_{\text{huge}}$+FT & &
44.26 & 54.24 & 48.75  & ~ &
44.99 & 55.35 & 49.64  & ~ &
6.86 & 53.61 & 12.16  \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\midrule
\multicolumn{17}{@{\hskip 0.11in}c}{\bf {AWA2 Dataset}}  \\ 
\midrule

\multirow{3}{*}{I-1k} & &
\multirow{2}{*}{CNN} & &

RN101 &&
75.48 & 59.56 & 66.58  & ~ &
75.95 & 54.76 & 63.87  & ~ &
69.26 & 56.03 & 61.95  \\

&& &&RN101+FT &&
84.81 & 58.44 & 69.20  & ~ &
77.74 & 59.95 & 69.14  & ~ &
83.43 & 47.66 & 60.66  \\ 

% && &&GoogleNet &&
% 69.08 & 55.17 & 61.35  & ~ &
% 71.51 & 53.22 & 62.22  & ~ &
% 73.36 & 47.63 & 57.76  \\

&& &&RN152 &&
84.48 & 60.01 & 70.17  & ~ &
\textbf{88.88} & 57.69 & 70.48  & ~ &
76.74 & 40.25 & 52.8  \\

\cmidrule{3-17}

&& \multirow{1}{*}{ViT} &&\cellcolor{gray!18}ViT$_{\text{large}}$&\cellcolor{gray!18}&
90.14 & 68.28 & 77.70  & ~ &
85.55 & 70.62 & 79.25  &\cellcolor{gray!18} ~ &
\cellcolor{gray!18}81.37 &\cellcolor{gray!18} \textbf{69.14} &\cellcolor{gray!18} \textbf{74.75}  \\

&& &&DeiT$_{\text{base}}$ && 
84.63 & 51.89 & 64.33  & ~ &
77.83 & 59.04 & 68.50  & ~ &
79.35 & 50.62 & 61.81  \\ 

&& &&ViTB16-DINO$^{\dag}$&& 
77.64 & 57.77 & 66.24  & ~ &
75.69 & 63.90 & 71.25  & ~ &
81.66 & 54.65 & 65.48  \\

\midrule

\multirow{3}{*}{I-21k} && \multirow{3}{*}{ViT} &&\cellcolor{gray!18} ViT$_{\text{large}}$ &\cellcolor{gray!18} &
\cellcolor{gray!18}\textbf{91.05} &\cellcolor{gray!18} \textbf{63.58} &\cellcolor{gray!18} \textbf{74.87}  &\cellcolor{gray!18} ~ &
\cellcolor{gray!18}88.69 &\cellcolor{gray!18} \textbf{70.75} &\cellcolor{gray!18} \textbf{80.40}  & ~ &
\textbf{78.32} & 59.21 & 67.44  \\

% && && ViT$_{\text{huge}}$ & &
% 88.85 & 60.79 & 72.19  & ~ &
% 85.68 & 60.95 & 72.25  & ~ &
% 75.57 & 53.24 & 62.47  \\

&& && ViT$_{\text{huge}}$+FT & &
68.23 & 61.63 & 64.76  & ~ &
80.69 & 60.76 & 69.32  & ~ &
75.23 & 60.10 & 66.82  \\

\bottomrule
\end{tabularx}

}

%\vspace{-0.05in}
\caption{
% Results of Embedding Based Methods using different features extracted from a diverse set of architecture types pretrained on ImageNet-1k (I-1k) and ImageNet-21k (I-21k)\cite{Imagenet}. These backbones were trained via: supervised and self-supervised (${\dag}$) learning. The bold numbers correspond to the highest scores per column, and the shaded rows correspond to the most performant image feature per method. +FT indicates the features were fine-tuned with the seen classes from the training set.
Results of Generative Based Methods using different features extracted from a diverse set of architecture types pretrained on ImageNet-1k (I-1k) and ImageNet-21k (I-21k). (${\dag}$) indicates self-supervised learning. The bold numbers and the shaded rows correspond to the highest scores and method. +FT indicates the features were fine-tuned with the seen classes from the training set. 
% The most performant visual features are extracted from a ViT$_{\text{huge}}$ pretrained on Imagenet21k and fine-tuned with the seen classes, using the tfVAEGAN method.
}
\label{tab:subset_generative_based}
\vspace{-0.1in}
\end{table*}


==> 04.5_subset_tables_disentanglement_noclip.tex <==
\begin{table*}[h!]
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}
\newcolumntype{Z}{>{\centering\arraybackslash}X}
\centering
\footnotesize
\setlength\tabcolsep{1pt}
\renewcommand{\arraystretch}{1.2}

\scalebox{0.87}{

\begin{tabularx}{\textwidth}{l c l c l c YYY c YYY}
\toprule

\multicolumn{13}{@{\hskip 0.11in}c}{\bf { CUB Dataset}}  \\ 
\midrule

{\multirow{2}{*}{\bf \shortstack{Dataset\\Pret. on}}}~ &~~~~&
{\multirow{2}{*}{\bf \shortstack{Arch\\ Type}}}~ &~~~~&
{\multirow{2}{*}{\bf Backbone}}~ &~~~~&
\multicolumn{3}{@{\hskip 0.11in}c}{\bf SDGZSL} &~~~~& 
\multicolumn{3}{@{\hskip 0.11in}c}{\bf FREE}  \\

\cmidrule{7-9}\cmidrule{11-13}

&& && && \textit{Seen} & \textit{Novel} & \textit{Harm.} 
&& \textit{Seen} & \textit{Novel} & \textit{Harm.} \\

\midrule

\multirow{3}{*}{I-1k} & &
\multirow{2}{*}{CNN} & &

RN101 &&
56.41 & 51.89 & 54.06  & ~ &
58.30 & 55.10 & 56.70  \\

&& &&RN101+FT &&
75.00 & 64.26 & 69.21  & ~ &
75.30 & 56.00 & 64.20  \\

% && &&GoogleNet &&
% 32.72 & 32.88 & 32.80  & ~ &
% 33.78 & 34.34 & 34.06  \\

&& &&RN152 &&
48.22 & 43.37 & 45.67  & ~ &
50.70 & 43.90 & 47.10  \\

\cmidrule{3-13}

&& \multirow{3}{*}{ViT} &&ViT$_{\text{large}}$&&
74.17 & 63.17 & 68.23  & ~ &
69.53 & 56.38 & 62.27  \\

&& &&DeiT$_{\text{base}}$ && 
62.91 & 54.40 & 58.35  & ~ &
61.80 & 43.80 & 51.27  \\ 

&& &&ViTB16-DINO$^{\dag}$&& 
68.72 & 64.25 & 66.41  & ~ &
73.70 & 53.46 & 61.97  \\

\midrule

\multirow{2}{*}{I-21k} && \multirow{2}{*}{ViT} && 
ViT$_{\text{large}}$ & &
79.55 & 64.37 & 71.16  & ~ &
73.07 & 52.91 & 61.37  \\

&& &&\cellcolor{gray!18} ViT$_{\text{huge}}$+FT &\cellcolor{gray!18} &
\cellcolor{gray!18}\textbf{79.68} &\cellcolor{gray!18} \textbf{73.27} &\cellcolor{gray!18} \textbf{76.34}  &\cellcolor{gray!18} ~ &
\cellcolor{gray!18}\textbf{80.57} &\cellcolor{gray!18} \textbf{69.71} &\cellcolor{gray!18} \textbf{74.75}  \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\midrule
\multicolumn{13}{@{\hskip 0.11in}c}{\bf { SUN Dataset}}  \\ 
\midrule

\multirow{3}{*}{I-1k} & &
\multirow{2}{*}{CNN} & &

RN101 &&
36.67 & 44.44 & 40.18  & ~ &
37.20 & 47.40 & 41.70  \\

&& &&RN101+FT &&
38.57 & 49.44 & 43.33  & ~ &
41.12 & 47.01 & 43.87  \\

% && &&GoogleNet &&
% 26.24 & 31.94 & 28.81  & ~ &
% 26.32 & 35.69 & 30.30  \\

&& &&RN152 &&
34.77 & 44.44 & 39.01  & ~ &
35.12 & 48.19 & 40.63  \\

\cmidrule{3-13}

&& \multirow{3}{*}{ViT} &&\cellcolor{gray!18}ViT$_{\text{large}}$&\cellcolor{gray!18}&
\cellcolor{gray!18}51.59 &\cellcolor{gray!18} 63.75 &\cellcolor{gray!18} \textbf{57.03}  &\cellcolor{gray!18} ~ &
\cellcolor{gray!18}\textbf{54.15} &\cellcolor{gray!18} 57.22 &\cellcolor{gray!18} \textbf{55.64}  \\

&& &&DeiT$_{\text{base}}$ && 
31.94 & 45.69 & 37.60  & ~ &
36.98 & 43.54 & 39.99  \\

&& &&ViTB16-DINO$^{\dag}$&& 
40.04 & 51.53 & 45.06  & ~ &
39.61 & 53.19 & 45.41  \\

\midrule

\multirow{2}{*}{I-21k} && \multirow{2}{*}{ViT} && ViT$_{\text{large}}$ & &
32.13 & \textbf{68.96} & 43.84  & ~ &
49.34 & \textbf{59.44} & 53.92  \\

&& && ViT$_{\text{huge}}$+FT & &
39.53 & 47.99 & 43.35  & ~ &
44.57 & 52.22 & 48.10  \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\midrule
\multicolumn{13}{@{\hskip 0.11in}c}{\bf { AWA2 Dataset}}  \\ 
\midrule

\multirow{4}{*}{I-1k} & &
\multirow{3}{*}{CNN} & &

RN101 &&
75.27 & 58.65 & 65.93  & ~ &
75.22 & \textbf{56.00} & 64.20  \\

&& &&RN101+FT &&
83.99 & 60.35 & 70.24  & ~ &
\textbf{87.66} & 47.56 & 61.67  \\

% && &&GoogleNet &&
% 71.62 & 54.53 & 61.91  & ~ &
% 72.03 & 49.45 & 58.64  \\

&& &&RN152 &&
79.08 & 68.38 & 73.34  & ~ &
86.78 & 50.13 & 63.55  \\

% && &&\cellcolor{gray!18}Inceptionv3$_{\text{adv}}$ &\cellcolor{gray!18}&
% 80.22 & 57.68 & 67.11  &\cellcolor{gray!18} ~ &
% \cellcolor{gray!18}85.38 &\cellcolor{gray!18} 51.71 &\cellcolor{gray!18} \textbf{64.41}  \\

\cmidrule{3-13}

&& \multirow{3}{*}{ViT} &&\cellcolor{gray!18}ViT$_{\text{large}}$&\cellcolor{gray!18}&
\cellcolor{gray!18}86.87 &\cellcolor{gray!18} \textbf{70.37} &\cellcolor{gray!18} \textbf{77.75}  & ~ &
87.29 & 48.14 & 62.06  \\

&& &&DeiT$_{\text{base}}$ && 
80.13 & 56.06 & 65.96  & ~ &
72.55 & 41.13 & 52.50  \\

&& &&ViTB16-DINO$^{\dag}$&& 
77.10 & 56.00 & 64.88  & ~ &
80.40 & 44.79 & 57.53  \\

\midrule

\multirow{2}{*}{I-21k} && \multirow{2}{*}{ViT} && ViT$_{\text{large}}$ & &
86.04 & 64.65 & 73.83  & ~ &
80.58 & 43.4 & 56.42  \\

&&  && ViT$_{\text{huge}}$+FT & &
76.94 & 58.43 & 66.42  & ~ &
82.36 & 43.10 & 56.59  \\

\bottomrule
\end{tabularx}

}

%\vspace{-0.05in}
\caption{Results of Generative Based Methods using different features extracted from a diverse set of architecture types pretrained on ImageNet-1k (I-1k) and ImageNet-21k (I-21k). (${\dag}$) indicates self-supervised learning. The bold numbers and the shaded rows correspond to the highest scores and method. +FT indicates the features were fine-tuned with the seen classes from the training set. }
\label{tab:subset_disentanglement_based}
\vspace{-0.1in}
\end{table*}





==> 05.2_methods.tex <==
% \subsection{Methods}

==> 05.3_figures.tex <==


\begin{figure}[h]
\centering
\includegraphics[width=.3\textwidth]{Images/gzsl_results_w_clip_finetuned_cub.pdf}\hfill
\includegraphics[width=.3\textwidth]{Images/gzsl_results_w_clip_finetuned_sun.pdf}\hfill
\includegraphics[width=.37\textwidth]{Images/gzsl_results_w_clip_finetuned_awa2.pdf}
\caption{Results when using features fine-tuned using the training seen classes with different GSZL methods. Overall, the generative-based methods (i.e., tfVAEGAN\cite{tfvaegan} and CADA-VAE\cite{CADA_VAE}) perform the best.}
\label{fig:finetuned_features_res}
\end{figure}




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

